Approximate Partial Order Reduction

We present a new partial order reduction method for reachability analysis of nondeterministic labeled transition systems over metric spaces. Nondeterminism arises from both the choice of the initial state and the choice of actions, and the number of executions to be explored grows exponentially with their length. We introduce a notion of $\varepsilon$-independence relation over actions that relate approximately commutative actions; $\varepsilon$-equivalent action sequences are obtained by swapping $\varepsilon$-independent consecutive action pairs. Our reachability algorithm generalizes individual executions to cover sets of executions that start from different, but $\delta$-close initial states, and follow different, but $\varepsilon$-independent, action sequences. The constructed over-approximations can be made arbitrarily precise by reducing the $\delta,\varepsilon$ parameters. Exploiting both the continuity of actions and their approximate independence, the algorithm can yield an exponential reduction in the number of executions explored. We illustrate this with experiments on consensus, platooning, and distributed control examples.

==> car.tex <==
automaton $\auto{Car Platoon}(N : \ioaNat)$
	variables
		$x:\Real^{2N}$ ;
		$m: \{c,a,b\}^{N}$;
	
	initially
		$\mbox{for each } i \in [N]$
			$m[i]:=$ choose $\{c,a,b\}$;
		
	transitions
		$\act{move}$
			pre 	true
			eff 	$m[0]:=$ choose $\{c,a,b\}$;
				$\mbox{for each } i \in [N] \setminus 0$
					$m[i]:= \left\{\begin{array}{ll} a & \mbox{ if } x[2(i-1)] - x[2i] >50\\ 
					b & \mbox{ if } x[2(i-1)] - x[2i] <30\\ c & \mbox{ else } \\ \end{array}\right.$;  
					$x:= Ax +  b_m$;




==> dcs.tex <==
automata $\auto{Linear}(n \in \naturals, N \in \naturals)$
	variables
		$x_i : \reals^n$;
		$\tilde x_i: \reals^n$;
		$y_i: \reals$
		$d :\booleans^N$;
	initially
		$x_i\in[-4,4]$ for each $i\in [n]$;
		$d_i := \mathit{false}$ for each $i\in[n]$;
	transitions
		$\act{a_i}$ for each $i\in[N]$ 
			pre 	$d_i = \false$
			eff 	$x := A_i x \ \wedge \ d_i := \true$;
		$\act{a_\bot}$
			pre   $\wedge_{i\in[N]} d_i$:
			eff	$d_i :=\mathit{false}$ for each $i\in[N]$;

==> linear.tex <==
automaton $\auto{Consensus}(n \in \naturals, N \in \naturals)$
	variables
		$x : \reals^n$
		$d :\booleans^N$
	initially
		$x[i]\in[-4,4]$ for each $i\in [n]$
		$d[i] := \mathit{false}$ for each $i\in[n]$
	transitions
		$\act{a_i}$ for each $i\in[N]$ 
			pre 	$\neg d_i$
			eff 	$x := A_i x \ \wedge \ d[i] := \true$
		$\act{a_\bot}$
			pre   $\wedge_{i\in[N]} d[i]$
			eff	$d[i] :=\mathit{false}$ for each $i\in[N]$

==> newalgo.tex <==
% !TEX root = main.tex

$A$ is the set of all actions, $\RT = \{\langle \tau, q, \dr \rangle\}$ is the table that contains all the representative traces $\tau$ such that the $\epsilon$-equivalence traces of $\tau$ has been considered, $q$ is the array of states visited through trace $\tau$ and $\dr$ is the corresponding bloating size. $RC$ is a set of states and $guardpartition(RC)$ returns a set of tuples $ \langle q_0, \delta, \EA \rangle$ such that $\EA$ is the set of actions enabled  for $B_{\delta}(q_c)$ and $\EA$ should be different in different tuples.




In this section, we present an algorithm to compute a ball centered at the final state of a potential execution $\xi$, such that the ball contains the final states of all ($\delta_0,\varepsilon$)-close executions of $\xi$.
Algorithm~\ref{por:algo:main} takes inputs of an execution $\xi = \exe{q_0,\tau}$, two parameters $\delta_0,\varepsilon \geq 0$, and a set of discrepancy functions $\{\beta_a\}_{a\in A}$. 
For each $t\in [len(\xi)]$, let $a$ be the $t$-th action of $\xi$ and $\tau$ be the prefix before $a$. 

The algorithm first finds the anchor position of each action on $\tau$.
Using the anchor positions, we can compute a sequence of representative radii $\{\delta_t\}_{t=1}^T$ inductively. 
Our computation guarantees that for each $t \in \{1,2,\dots,T\}$, 
the length $t$ prefixes of $\xi$ is a ($\delta_0,\varepsilon,\delta_t$)-representative potential execution.

%\begin{wrapfigure}{R}{5cm}
\begin{algorithm}
\caption{Generalization($\xi, \delta_0, \varepsilon, \{\beta_a\}_{a\in A}$)}
\label{por:algo:main}
\begin{algorithmic}[1]
%\Procedure{Bloat}{$\xi, \delta_0, \varepsilon, \beta$}
   \State $\beta \gets \max\{\beta_a\}$;
%   \State $\R \gets \B_{\delta_0}(\xi(0))$;
   \State $T\gets len(\xi)$;
   \For{$t \in [T]$}
   	\State
   	//{\em let $\tau a$ be the length ($t+1$) prefix of $\trace \xi$}
%   	\State $\eta \gets$ maximum suffix of $\mathit{prefix}_t(\trace{\xi})$  such that $\eta\mysim\varepsilon Trace(\xi,t)$ \label{ln:eta}
	\State \chuchu{$k\gets\mathit{anchor(\tau, a, \epsilon)}$;}
	%the position of the last action $b$ on $\tau$ such that $b\not\mysim\varepsilon a$
   	\If{$k = t$} 
		\State $\delta_{t+1}\gets \beta_{a}(\delta_t)$;
		\label{ln:case1}
		%\Comment{$a$ cannot be swapped}
	\Else  
		%\State $\beta \gets \max_{a\in \tau}\{\beta_a\}$
		\State $\delta_{t+1}\gets \beta_a(\delta_t) +  \gamma_{t-k-1}(\varepsilon)$;	
		\label{ln:case2}
		%\Comment{$a$ can be swapped to a position $>k$}
	\EndIf
   \EndFor
   \State \Return $ \B_{\delta_{T}}(\xi(T))$;
%\EndProcedure  
\end{algorithmic}
\end{algorithm}
%\end{wrapfigure}

%\subsection{Algorithm analysis}

%\begin{proposition}
%Fix any $t\in[len(\xi) -1]$ and any $\xi'$ that is ($\delta_0,\varepsilon$)-close to the 
%length $t$ prefix of $\xi$.
%Let $\tau, a, k$ be defined as in line 4-5 of the algorithm.
%\end{proposition}
%\begin{proof}
%For any $t\in[len(\xi) - 1]$, let $\tau\in A^t$ be the length $t$ prefix of $\trace{\xi}$ and $a\in A$ be
%the ($t+1$)th action on 
%\end{proof}
We will establish the correctness of Algorithm~\ref{por:algo:main}.
First, we will show that the sequence of $\{\delta_t\}_{t=1}^T$ is valid representative radii for the prefixes of $\xi$.
\begin{lemma}
\label{por:lem:sound}
For any $t \leq len(\xi)$, the $t$ length prefix of $\xi$ is a $(\delta_0,\varepsilon,\delta_t)$-representative execution.
\end{lemma}


\begin{proof}
For any $t\leq len(\xi)$, 
We prove the lemma by induction on $t$.\\	
{\bf Base:} For $t = 0$, the length $0$ prefix of $\xi$ is a single state $q_0$. 
Any $\xi'$ ($\delta_0,\varepsilon$)-close to $q_0$ is also a single state $q_0'$
with $q'_0 \in \B_{\delta_0}(q_0)$. Hence the lemma holds for $t=0$.\\
{\bf Induction:} Suppose the lemma holds for any prefix of $\xi$ with length at most $t < len(\xi)$.
We will prove it for the length $t+1$ prefix of $\xi$.
Let $q_0$ be the initial state of $\xi$, $\tau$ be the length $t$ prefix of $\trace{\xi}$, and $a\in A$ is the ($t+1$)th action.
Then $\xi_{t+1} = \exe{q_0, \tau a}$ is the length $t+1$ prefix of $\xi$.
The execution $\xi_{t+1}$ is illustrated in Figure~\ref{fig:exes_algo}.
\chuchu{Fix any $\xi'$ that is ($\delta_0,\varepsilon$)-close to $\xi_{t+1}$.}
From Proposition~\ref{por:prop:perm_loc}, $\xi'.\lstate.L = \xi_{t+1}.\lstate.L$.
It suffice to prove that $|\xi'.\lstate.X - \xi_{t+1}.\lstate.X| \leq \delta_{t+1}$. 

\begin{figure}
	\centering
	\includegraphics[width=0.4\textwidth]{algo.png}
	\caption{Potential executions $\xi_{t+1}$, $\xi'$, and $\xi''$ constructed by swapping action $a$ in $\xi'$.}
	\label{fig:exes_algo}
\end{figure}

Since $\trace{\xi'} \myequiv \varepsilon \tau a$, action $a$ is in the sequence $\trace{\xi'}$.
Partitioning $\trace{\xi'}$ on the last occurrence of $a$, we get $\trace{\xi'} =\phi a \eta$ for some $\phi,\eta\in A^*$ with $a\not\in \eta$.
Since $k$ is the anchor position, from Definition~\ref{def:anchor}, the position of the  last occurrence of $a$ on $\trace{\xi'}$ is at least $k$.
Hence we have $len(\phi) \geq k$ and $len(\eta) = t - len(\phi) \leq t-k$.
\chuchu{We construct another potential execution $\xi'' = \exe{q'_0, \phi\eta a}$ with the same initial state as $\xi'$.
The executions $\xi,\xi'$ and $\xi''$ are illustrated in Figure~\ref{fig:exes_algo}.}
%

%
From the inductive hypothesis, the length $t$ prefix of $\xi_{t+1}$, which is the execution
$\xi_t = q_0,\tau,a_t$ in the figure is an ($\delta_0, \varepsilon, \delta_{t}$)-representative execution.
We note that the length $t$ prefix $\xi''$ is ($\delta_0,\varepsilon$)-close to $\xi_t$. 
Therefore, $|q_t.X - q_t''.X| \leq \delta_t$. Using the discrepancy function of action $a$, we have
\begin{equation}
\label{por:eq:algo1}
|q_{t+1}.X - q_{t+1}''.X| \leq \beta_a(|q_t.X - q_t''.X|) \leq \beta_a(\delta_t).
\end{equation}
We will quantify the distance between $\xi'$ and $\xi''$.
There are two cases: \\
(i) If $k = t$ and line~\ref{ln:case1} is executed.
Then, $len(\eta) \leq t-k = 0$, that is, $\eta$ is an empty string. 
Hence, $\xi'$ and $\xi''$ are indeed identical and $q'_{t+1} = q''_{t+1}$. 
Thus from~\eqref{por:eq:algo1},
\[
|q_{t+1}.X-q'_{t+1}.X| = |q_{t+1}.X - q_{t+1}''.X| \leq \beta_a(\delta_t).
\] 
Therefore if $\delta_{t+1}$ is computed by line~\ref{ln:case1}, the lemma holds for the length $t+1$ prefix of $\xi$.
(ii) Otherwise $k < 0$ and line~\ref{ln:case2} is executed. 
From Lemma~\ref{por:lem:insert}, we can bound the distance between $\xi'$ and $\xi''$ as
%\[
$|q_{t+1}'.X-q_{t+1}''.X| \leq \gamma_{len(\eta)-1}(\varepsilon) \leq \gamma_{t-k-1}(\varepsilon).$
%\]
Combining with~\eqref{por:eq:algo1}, we get
\[
|q_{t+1}.X-q'_{t+1}.X| \leq |q_{t+1}.X-q'_{t+1}.X| + |q_{t+1}.X-q'_{t+1}.X| \leq 
\beta_a(\delta_t) + \gamma_{t-k-1}(\varepsilon).
\]
Therefore if $\delta_{t+1}$ is computed by line~\ref{ln:case2}, the lemma holds for the length $t+1$ prefix of $\xi$, which completes the proof.
\qed
\end{proof}

Using this lemma and Proposition~\ref{por:prop:gamma}, we establish the soundness and the precision of the reachability algorithm (see~\cite{HM:TACAS-full} for proofs).
\begin{theorem}[Soundness]
\label{por:thm:sound}
For any execution $\xi'$ such that $\xi'$ is ($\delta_0,\varepsilon$)-close to $\xi$,
 the last state of $\xi'$ is in the returned set  $\ball{\delta_T}{\xi(T)}$.
\end{theorem}
%\begin{proof}
%From Lemma~\ref{por:lem:sound}, $\xi$ is a ($\delta_0,\varepsilon,\delta_T$)-representative potential execution. From Definition~\ref{por:def:represent}, for any potential execution $\xi'$ that is ($\delta_0,\varepsilon$)-close to $\xi$, we have $\xi'.\lstate\in \ball{\delta_T}{\xi(T)}$.
%\end{proof}

%In the following theorem, we show that the radius $\delta_T$ can be made arbitrarily small for small enough initial radius $\delta_0$ and the approximation parameter $\varepsilon$.
\begin{theorem}[Precision]
\label{por:thm:complete}
For any $t \leq len(\xi)$, as $\delta_0 \rightarrow 0$ and $\varepsilon \rightarrow 0$, the size of radius $\delta_T$ goes to 0.
\end{theorem}
%\begin{proof}
%From Proposition~\ref{por:prop:gamma}, 
%for any $n$, $\gamma_n(\varepsilon)\rightarrow 0$ as $\varepsilon \rightarrow 0$.
%From Definition~\ref{por:def:discrep}, for any $\delta_t$ and discrepancy function $\beta$, $\beta(\delta_t) \rightarrow 0$ as $\delta_t\rightarrow 0$.
%Therefore, either line 6 or line 8 in Algorithm~\ref{por:algo:main} is executed, $\delta_{t+1} \rightarrow 0$ as $\delta_t\rightarrow 0$ and $\varepsilon\rightarrow 0$.
%Iteratively applying this observation leads that, $\delta_T\rightarrow 0$ as $\delta_0\rightarrow 0$ and $\varepsilon \rightarrow 0$.
%Therefore the theorem holds. 
%\end{proof}
%In the following 
The precision theorem, states that the radius $\delta_T$ of the reachset at time $T$ can be made arbitrarily small with a small enough choice of initial radius $\delta_0$ and the approximation parameter $\varepsilon$.
%For an execution $\xi$ of length $n$,
%the worst case time complexity of Algorithm~\ref{por:algo:main} is $O(n^3)$, 
%since finding the anchor position can take at most $O(n^2)$ time.
If all actions in $\xi$ are mutually approximately independent, the algorithm can over-approximate the final states of  $O(n!)$ executions which can lead to a dramatic savings in reach set computation.
%In the next section, we will use Algorithm~\ref{por:algo:main} as a subroutine to compute an over-approximation  of the reach set of a labeled transition system in a more or less standard fashion.


\chuchu{
\begin{example}
Consider a car running on a straight road. Between each time step the acceleration or declaration is considered to be a constant number, then the system can be written as 
\[
\begin{bmatrix}
s[t+1] \\
v[t+1]
\end{bmatrix} = 
\begin{bmatrix}
1 & 0.1 \\
0 & 1
\end{bmatrix}
\]
\end{example}
}
\section{Reachset Over-approximation with Partial Order Reduction}
\label{por:sec:reach_algo}


%In Section~\ref{por:sec:general}, we presented a 
Using the  \chuchu{$generalization()$} function that over-approximates the reach set of a group of ($\delta,\varepsilon$)-close potential executions using a single potential execution, we present an algorithm to compute an over-approximation of the reach set of a labeled transition system.
%
Recall that  for any set of initial states $S\subseteq \Theta$ and time bound $T\geq 0$, $\execs{S,T}$ is the set of executions from $S$ of length $T$, and $\traces{S, T}$ is the set of action sequences of these executions.
%
In concurrent systems, even  singleton initial can set  the size of $\traces{S, T}$ growing exponentially with $T$.
Partial order reduction methods reduce the number of action sequences needed to be explored. 
These methods exploit the equivalence relation on the set of action sequences and divide  
$\traces{S, T}$ into equivalence classes.
Then, checking a representative action sequence suffice to cover the whole equivalence class.
We formally define the set of representative action sequences.
%%

\begin{definition}
\label{por:def:repseq}
For any time bound $T\geq 0$, any equivalence relation $\myequiv \varepsilon$ on the set of length $T$ action sequences $A^T$, and any subset of initial states $S\subseteq Q$,
the set of {\em $T$-representative action sequences from $S$\/} is the quotient of the set $\traces{S, T}$ by the equivalence relation $\myequiv\varepsilon$.
\end{definition}
% a set $\T\subseteq \traces{S, T}$ such that
% \begin{enumerate}[(i)]
% \item any pair of action sequences in $\T$ are not $\varepsilon$-independent, and 
% \item an action sequence $\tau\in \T$ is a $T$-representative sequence iff there exists a action sequence $\tau'\in \traces{S, T}$ such that $\tau\myequiv\varepsilon\tau'$.
% \end{enumerate}
That is, for any length $T$ execution $\xi$ starting from $S$, there exists a unique $T$-representative action sequence $\tau\in\T$, such that $\tau \myequiv\varepsilon \trace{\xi}$.
Over the past few decades, various methods have been proposed to compute the representative action sequences for finite-state machines~\cite{clarke1999model,yang2008efficient}.
%Roughly, there are two main classes of methods that have been proposed.
%For each state $q$, the {\em ample/persistent set} techniques select an ample set as a subset of enabled actions from $q$, where the missing actions are independent to those actions in the ample set~\cite{clarke1999model}.
%Then execution sequences that take actions from the ample sets are the representatives for equivalent classes.
%In contrast, the {\em sleep set} techniques decide which action to explore on-the-fly~\cite{yang2008efficient}. 
%The technique maintains a sleep set as a set of actions that should not be explored immediately and update the set based on the independence relation along the execution.
%We can use any of these methods in the reachability algorithm.
%\sayan{So, the approximations dont affect this computation?}
\zhenqi{Computing $T$-representative action sequences for infinite-state system is a non-trivial problem, however it is out of the scope of this paper.}
%\subsection{Reach Set Over-approximation}

%We propose an algorithm to compute an over-approximation of $\reach{}{\Theta, T}$. 
Given a labeled transition system, an approximation parameter $\varepsilon \geq 0$, a partition parameter $\delta > 0$, a time bound $T>0$, and a set of \chuchu{discrepancy functions} $\{\beta_a\}_{a\in A}$, the following algorithm computes an over-approximation of reach set at time $T$.
%
We first compute a $\delta$-cover $Q_0$ of the initial set $\Theta$ such that $\ball{\delta}{Q_0} \supseteq \Theta$.
Then, in line~\ref{por:ln:repseq}, we compute the $T$-representative action sequences from each cover $\ball{\delta}{q_0}$.
Then, we use the algorithm \chuchu{$Generalization()$} to compute a ball $\R'$ that over-approximate the set of states reached by a group of executions from a cover following equivalent action sequences.
The algorithm returns $\R$, the union of these balls $\R'$.

%\sayan{(a)the numbering of the algorithms should be 1, 2, ..
%	(b) what are the input parameters of the algorithm beyond $\Theta$ and $T$? $\epsilon$? Let us include them in the name in the caption and also explicitly in the discussion. }

%\begin{minipage}{5cm}
\begin{algorithm}[th!]
\caption{Reachability algorithm to over-approximate $\reach{}{\Theta,T}$}
\label{por:algo:reach}
\begin{algorithmic}[1]
\State $Q_0 \gets \delta$-$cover(\Theta)$; $\R\gets \emptyset$;
\For{$q_0\in Q_0$}
	\State $\T\gets \traces{\ball{\delta}{q_0}} \slash \myequiv{\varepsilon}$; \label{por:ln:repseq}
	\For{$\tau\in \T$}
		\State $\R' \gets Generalization(\exe{q_0,\tau}, \delta, \varepsilon,\{\beta_a\}_{a\in A})$;
		\label{por:ln:general}
		\State $\R \gets \R \cup \R'$;
	\EndFor
\EndFor
\State \Return $\R$;  
\end{algorithmic}
\end{algorithm}
%\end{minipage}
	
%\subsection{Analysis of the Algorithm}
We  show that, for any $T\geq 0$, the set $\R$ over-approximate the reach set of the system at time $T$. Also, the over-approximation can be made precise (see~\cite{HM:TACAS-full} for full proofs). 
%The proof of the precision theorem follows Theorem~\ref{por:thm:complete} and the definition of $T$-representative action sequences.

\begin{theorem}[Soundness]
Set $\R$ returned by Algorithm~\ref{por:algo:reach}, satisfies $\reach{}{\Theta,T} \subseteq \R$.
\end{theorem}
%\begin{proof}
%Fixed any $\xi \in \execs{\Theta, T}$, it suffice to show that $\xi(T)\in \R$.
%Since $\xi(0)\in \Theta$ and $Q_0$ is a $\delta$-cover,
%there exists a $q_0\in Q_0$ such that $\xi(0)\in \ball{\delta}{q_0}$.
%For this $q_0$, let $\T$ be the $T$-presentative action sequences from $\ball{\delta}{q_0}$ computed in line~\ref{por:ln:repseq} .
%From Definition~\ref{por:def:repseq}, there must be a representative action sequence $\tau \in \T$ such that $\tau \myequiv \varepsilon \trace{\xi}$.
%Since $\xi$ is ($\delta,\varepsilon$)-close to $\exe{q_0,\tau}$,
%from Theorem~\ref{por:thm:sound}, the $\R'$ computed using $Generalization()$ guarantees that
%$\xi.\lstate\in \R$.
%Therefore the theorem holds.
%\end{proof}


\begin{theorem}[Precision]
For any $r>0$, there exist $\delta,\varepsilon>0$ such that, the set $\R$ computed by Algorithm~\ref{por:algo:reach} satisfies
$\R\subseteq\ball{r}{\reach{}{\Theta,T}}$.
\end{theorem}
%\begin{proof}
%Fix arbitrary $r>0$.
%The set $\R$ is a union of balls $\R'$ computed in line~\ref{por:ln:general}.
%Fix any such $\R'$ centered at the last state of potential execution $\xi = \exe{q_0,\tau}$.
%It suffices to show that $\R'$ satisfies $\R'\subseteq\ball{r}{\reach{}{\Theta,T}}$ for small enough $\delta$ and $\varepsilon$.
%
%Since $\tau\in \T$ is a $T$-representative action sequence from the initial set $\ball{\delta}{q_0}$, from Definition~\ref{por:def:repseq}, there exists an action sequence $\tau' \in \traces{\ball{\delta}{q_0}, T}$ such that $\tau$ and $\tau'$ are $\varepsilon$-equivalent.
%Hence, there is an execution $\xi'\in \execs{\ball{\delta}{q_0}, T}$ from the ball $\ball{\delta}{q_0}$ following the action sequence $\tau'$.
%By the definition of reach set, we have $\xi'.\lstate\in \reach{}{\Theta,T}$.
%On the other hand, $\xi'$ is ($\delta,\varepsilon$)-close to the potential execution $\xi$.
%From Theorem~\ref{por:thm:sound}, $\xi'.\lstate$ is in the ball $\R'$.
%That is, the ball $\R'$ and the reach set $\reach{}{\Theta,T}$ intersect at the state $\xi'.\lstate$.
%
%From Theorem~\ref{por:thm:complete}, the radius of $\R'$ can be made arbitrarily small as $\delta$ and $\varepsilon$ go to $0$.
%We chose small enough $\delta$ and $\varepsilon$, such that the radius of $\R'$ is less than $r/2$.
%Therefore, the ball $\R'$ is contained in the radius $r$ ball of the reach set $\ball{r}{\reach{}{\Theta,T}}$.
%\end{proof}

%In this section, we proposed an algorithm to over-approximate the reach set of label transition systems.
%In addition, we showed that the computation can be made arbitrarily precise.
%We will apply our method to verification of a linear transition system and a temperature control system.
%
%With the bloating algorithm presented above to generalize a single execution, 
%we are able to present an algorithm that computes over-approximations of reach set of an infinite state transition system. The key idea of the reachability algorithm is to generate exactly one execution for each equivalent class of executions, and then generalize this representative execution to over-approximate all equivalent executions.
%
%\begin{algorithm}
%\caption{Reachability algorithm}
%\label{alg:main}
%\begin{algorithmic}[1]
%\State $Q_0 \gets r$-$Partition(\Theta)$;
%\State $\R\gets \emptyset$;
%\For{$q_0\in Q_0$}
%	\State $\R \gets \R \cup$Explore($\langle \rangle, q_0, T$);
%\EndFor
%\State \Return $\R$;
%
%\Procedure{Explore}{$\xi, q, t$}
%\State $E \gets \{a\in enabled(q) \ |\ a < Trace(\xi, len(\xi) - 1)\}$;
%   \If{$E = \emptyset \vee t < 0$}
%      \State \Return Bloat($\xi$);
%   \EndIf
%   \State $\R \gets \emptyset$;
%   \For{$a\in E$}
%   	\State $\R \cup$Explore($\xi a, a(q), t - 1$);
%   \EndFor
%   \State \Return $\R$;
%\EndProcedure
%  
%\end{algorithmic}
%\end{algorithm}
%
%\begin{theorem}[Soundness]
%The returned set $\R$ of Algorithm~\ref{alg:main} contains all execution from $\Theta$ with length no more than $T$.
%\end{theorem}
%
%\begin{theorem}[Completeness]
%As $\varepsilon$ and $r$ converges to 0, $\R$ converges to the exact reach set.
%\end{theorem}

==> roomheating.tex <==
automaton $\auto{Roomheating}(N : \ioaNat)$
	variables
		$x:\Real^N$ initially $x[i]:=60$;
		$y:\Real^N$ initially $y[i]:= 60$;
		$d : \Bool^N$ initially $d :=  \false^N$;
		$m: \Bool^N$  initially $m :=  \false^N$;
		
	transitions
		$\act{on_i}$, for $i\in [N]$
			pre 	$! d[i] \wedge y[i] <= 72$
			eff 	$x:= W_hx + b_h +  C_h m$; 
					$d[i] := \true \wedge m[i] := \true$;

		$\act{off_i}$, for $i\in [N]$
			pre 	$! d[i] \wedge y[i]  >= 68$
			eff 	$x:= W_hx + b_h +  C_h m$; 
					$d[i] := \true \wedge m[i] := \false$;

						
		$\act{flow}$
			pre	$\wedge_{i\in [N]} d_i $
			eff	$x := W_T x + b_T + C_T m$;
					$d[i] := \false$ for each $i\in[N]$;
					$y:= x$;


